Encoding and Topological Computation on Textiles

A textile structure is a periodic arrangement of threads in the thickened plane. A topological classification of textile structures is harder than for classical knots and links that are non-periodic and restricted to a bounded region. The first important problem is to encode all textile structures in a simple combinatorial way. This paper extends the notion of the Gauss code in classical knot theory, providing a tool for topological computation on these structures. As a first application, we present a linear time algorithm for determining whether a code represents a textile in the physical sense. This algorithm, along with invariants of textile structures, allowed us for the first time to classify all oriented textile structures woven from a single component up to complexity five.

==> SMI Realizability of Textiles/SMI_Cover.tex <==

\usepackage{amsmath}

\begin{document}
Dear Sir/Madam

We are pleased that our paper has been conditionally accepted for SMI2020, and would like to thank the reviewers for the time they have taken in providing such detailed analysis of our work.

 In the resubmitted paper, major textual changes are given in blue
\smallskip

The attached table clarifies some of the changes and answers any accompanying queries. Some points that address multiple reviewer comments are detailed below:

 \begin{itemize}
 \item Algorithm $16$ is given in high level description only. Algorithm $17$ contained an error - the step that appends a completed cycle to $CYC$  should be inside the outer while loop. We believe that this corrects other issues - the algorithm now breaks if a cycle requires an already used pair. 
 \item Polynomials were calculated for all valid codes after reduction - they are not shown in the paper where they were identical to other knots.
 \item Textiles are shown up to ambient isotopy (and, for shortness, reversal of orientation). Not all symmetries or exchanges of over- and undercrossings are isotopies in this sense. 
 \end{itemize}
 \smallskip
 
 Reviewers  commented more generally on potential extensions to the paper:
 \begin{itemize}
\item Both multi-component and higher complexity textiles generate potentially very large input sets. Currently our code generates all codes, tests for validity and performs further reductions as described in the paper. We are adjusting this so that redundant codes are not generated initially. 
\item We are developing approaches to automating some of the manual steps involved in detecting non-proper and isotopic textiles. 
\item Detection of non-proper textiles in particular is only trivial in some cases. We are investigating a conjecture that a textile is non-proper if and only if one of the cycles arising in the algorithm contains two oriented edge symbols that attach to an edge of the diagram: this is clear in one direction, but the converse is harder to prove. 
 \end{itemize}
 
 We hope that this clarifies all key points. 
 \medskip
 
 Warm Regards
 \medskip 
 
 Matt Bright \& Vitaliy Kurlin.
 
 \newpage
 
 \begin{tabular}{|p{7 cm}|p{7 cm}|}
 \hline
\textbf{Comment} & \textbf{Response}\\
 \hline
 \hline
In Definition $6$, I think "each symbol i appears exactly once" is missing & This has now been added\\
 \hline
Definition $7$: "(possibly infinitely many) lines or circles": Is there any other possibility than zero or infinity? Can You construct textiles with only a finite number $n>0$ of lines or circles? & We may have any (countable) number of lines or circles. The definition has been updated to 'countably many' to ensure that this is clear\\
\hline
It is not clear to me, if the projection of the boundary curves of the strip in Definition 7 (page 3, line 31) have to coincide in the projection to $\mathbb{R}^2$. & This is indeed a requirement and we have clarified in the text.\\
\hline
in Definition $6$, the overcrossings are labeled by a superscript sign; is there any good reason to change this to labels for undercrossings in Definition $8$? This should be consistent. & This is an error in definition $6$ - in both Gauss and textile codes superscripts occur at undercrossings.\\
\hline
In Definition 9, I needed some time to realize that "proper" here is defined for "abstract code", and that this does not necessarily match "proper textiles". & The definition of 'proper code' was an artefact of a previous draft of the paper. It is not necessary and does cause confusion  - we have removed it in the resubmitted draft.\\
\hline
For some reason, I couldn't understand Fig 3 until I consulted an external reference for a definition of Reidemeister moves.& A more detailed explanation is now provided in the caption, and similarly for crossing conventions.\\
\hline
Page 3, L31: "such that $\mathbb{R} x \{+-1\}$ ..." I did not understand this condition or why it is necessary & This ensures that the ribbon is inserted such that it spans the height of the thickened plane.\\
\hline
Codes of complexity 5 with 2 crossings were found to represent textiles given by codes of complexity 4 via a homeomorphism"& We classify textiles up to embeddings in a fixed torus - this homeomorphism is not permitted.\\
\hline
...it seems polynomials are given only for the structures in column 6, after structures manually determined to be isotopic to others were pruned. & While we give polynomials only for distinct structures, they were calculated for all structures after reduction.\\
\hline
 \end{tabular}


\end{document}

==> SMI_Cover.tex <==

\usepackage{amsmath}

\begin{document}
Dear Sir/Madam

We are pleased that our paper has been conditionally accepted for SMI2020, and would like to thank the reviewers for the time they have taken in providing such detailed analysis of our work.

 In the resubmitted paper, major textual changes are given in blue
\smallskip

The attached table clarifies some of the changes and answers any accompanying queries. Some points that address multiple reviewer comments are detailed below:

 \begin{itemize}
 \item Algorithm $16$ is given in high level description only. Algorithm $17$ contained an error - the step that appends a completed cycle to $CYC$  should be inside the outer while loop. We believe that this corrects other issues - the algorithm now breaks if a cycle requires an already used pair. 
 \item Polynomials were calculated for all valid codes after reduction - they are not shown in the paper where they were identical to other knots.
 \item Textiles are shown up to ambient isotopy (and, for shortness, reversal of orientation). Not all symmetries or exchanges of over- and undercrossings are isotopies in this sense. 
 \end{itemize}
 \smallskip
 
 Reviewers  commented more generally on potential extensions to the paper:
 \begin{itemize}
\item Both multi-component and higher complexity textiles generate potentially very large input sets. Currently our code generates all codes, tests for validity and performs further reductions as described in the paper. We are adjusting this so that redundant codes are not generated initially. 
\item We are developing approaches to automating some of the manual steps involved in detecting non-proper and isotopic textiles. 
\item Detection of non-proper textiles in particular is only trivial in some cases. We are investigating a conjecture that a textile is non-proper if and only if one of the cycles arising in the algorithm contains two oriented edge symbols that attach to an edge of the diagram: this is clear in one direction, but the converse is harder to prove. 
 \end{itemize}
 
 We hope that this clarifies all key points. 
 \medskip
 
 Warm Regards
 \medskip 
 
 Matt Bright \& Vitaliy Kurlin.
 
 \newpage
 
 \begin{tabular}{|p{7 cm}|p{7 cm}|}
 \hline
\textbf{Comment} & \textbf{Response}\\
 \hline
 \hline
In Definition $6$, I think "each symbol i appears exactly once" is missing & This has now been added\\
 \hline
Definition $7$: "(possibly infinitely many) lines or circles": Is there any other possibility than zero or infinity? Can You construct textiles with only a finite number $n>0$ of lines or circles? & We may have any (countable) number of lines or circles. The definition has been updated to 'countably many' to ensure that this is clear\\
\hline
It is not clear to me, if the projection of the boundary curves of the strip in Definition 7 (page 3, line 31) have to coincide in the projection to $\mathbb{R}^2$. & This is indeed a requirement and we have clarified in the text.\\
\hline
in Definition $6$, the overcrossings are labeled by a superscript sign; is there any good reason to change this to labels for undercrossings in Definition $8$? This should be consistent. & This is an error in definition $6$ - in both Gauss and textile codes superscripts occur at undercrossings.\\
\hline
In Definition 9, I needed some time to realize that "proper" here is defined for "abstract code", and that this does not necessarily match "proper textiles". & The definition of 'proper code' was an artefact of a previous draft of the paper. It is not necessary and does cause confusion  - we have removed it in the resubmitted draft.\\
\hline
For some reason, I couldn't understand Fig 3 until I consulted an external reference for a definition of Reidemeister moves.& A more detailed explanation is now provided in the caption, and similarly for crossing conventions.\\
\hline
Page 3, L31: "such that $\mathbb{R} x \{+-1\}$ ..." I did not understand this condition or why it is necessary & This ensures that the ribbon is inserted such that it spans the height of the thickened plane.\\
\hline
Codes of complexity 5 with 2 crossings were found to represent textiles given by codes of complexity 4 via a homeomorphism"& We classify textiles up to embeddings in a fixed torus - this homeomorphism is not permitted.\\
\hline
...it seems polynomials are given only for the structures in column 6, after structures manually determined to be isotopic to others were pruned. & While we give polynomials only for distinct structures, they were calculated for all structures after reduction.\\
\hline
 \end{tabular}


\end{document}
